Matrix-Valued Measures and Wishart Statistics for Target Tracking Applications

Ensuring sufficiently accurate models is crucial in target tracking systems. If the assumed models deviate too much from the truth, the tracking performance might be severely degraded. While the models are usually defined using multivariate conditions, the measures used to validate them are most often scalar-valued. In this paper, we propose matrix-valued measures for both offline and online assessment of target tracking systems. Recent results from Wishart statistics, and approximations thereof, are adapted and it is shown how these can be incorporated to infer statistical properties for the eigenvalues of the proposed measures. In addition, we relate these results to the statistics of the baseline measures. Finally, the applicability of the proposed measures are demonstrated using two important problems in target tracking: (i) distributed track fusion design; and (ii) filter model mismatch detection.

==> fig/data__results_model_mismatch_check_nis.tex <==

\drawlambda[thick,clrlambdamax,dashed]\plotcommand{(2,6.832)(3,5.387)(4,4.600)(5,4.096)(6,3.740)(7,3.477)(8,3.270)(9,3.103)(10,2.965)(11,2.850)(12,2.750)(13,2.664)(14,2.589)(15,2.522)(16,2.463)(17,2.409)(18,2.360)(19,2.316)(20,2.275)(21,2.238)(22,2.204)(23,2.172)(24,2.142)(25,2.114)(26,2.088)(27,2.064)(28,2.042)(29,2.020)(30,2.000)(31,1.980)(32,1.962)(33,1.945)(34,1.928)(35,1.913)(36,1.897)(37,1.883)(38,1.870)(39,1.856)(40,1.844)(41,1.832)(42,1.820)(43,1.809)(44,1.799)(45,1.788)(46,1.778)(47,1.769)(48,1.759)(49,1.750)(50,1.742)(51,1.733)(52,1.725)(53,1.717)(54,1.709)(55,1.702)(56,1.695)(57,1.688)(58,1.681)(59,1.675)(60,1.668)};
\drawlambda[thick,black,dashed]\plotcommand{(2,0.052)(3,0.113)(4,0.168)(5,0.216)(6,0.256)(7,0.291)(8,0.321)(9,0.348)(10,0.372)(11,0.393)(12,0.412)(13,0.429)(14,0.445)(15,0.460)(16,0.473)(17,0.485)(18,0.497)(19,0.508)(20,0.518)(21,0.527)(22,0.536)(23,0.544)(24,0.552)(25,0.560)(26,0.567)(27,0.574)(28,0.580)(29,0.586)(30,0.592)(31,0.598)(32,0.603)(33,0.608)(34,0.613)(35,0.618)(36,0.623)(37,0.627)(38,0.632)(39,0.636)(40,0.640)(41,0.644)(42,0.647)(43,0.651)(44,0.654)(45,0.658)(46,0.661)(47,0.664)(48,0.667)(49,0.670)(50,0.673)(51,0.676)(52,0.679)(53,0.682)(54,0.684)(55,0.687)(56,0.689)(57,0.692)(58,0.694)(59,0.696)(60,0.699)};
\drawlambda[thick,black,dashed]\plotcommand{(2,3.715)(3,3.091)(4,2.744)(5,2.519)(6,2.358)(7,2.237)(8,2.142)(9,2.064)(10,2.000)(11,1.945)(12,1.898)(13,1.857)(14,1.821)(15,1.789)(16,1.760)(17,1.734)(18,1.711)(19,1.689)(20,1.669)(21,1.651)(22,1.634)(23,1.618)(24,1.604)(25,1.590)(26,1.577)(27,1.565)(28,1.553)(29,1.543)(30,1.533)(31,1.523)(32,1.514)(33,1.505)(34,1.497)(35,1.489)(36,1.481)(37,1.474)(38,1.467)(39,1.460)(40,1.454)(41,1.448)(42,1.442)(43,1.436)(44,1.431)(45,1.426)(46,1.420)(47,1.416)(48,1.411)(49,1.406)(50,1.402)(51,1.397)(52,1.393)(53,1.389)(54,1.385)(55,1.381)(56,1.378)(57,1.374)(58,1.370)(59,1.367)(60,1.364)};
\drawlambda[thick,clrlambdamin,dashed]\plotcommand{(2,0)(3,0.002)(4,0.010)(5,0.025)(6,0.044)(7,0.065)(8,0.086)(9,0.107)(10,0.127)(11,0.146)(12,0.164)(13,0.181)(14,0.197)(15,0.212)(16,0.227)(17,0.241)(18,0.254)(19,0.266)(20,0.278)(21,0.289)(22,0.300)(23,0.310)(24,0.320)(25,0.329)(26,0.338)(27,0.347)(28,0.355)(29,0.363)(30,0.371)(31,0.378)(32,0.385)(33,0.392)(34,0.399)(35,0.405)(36,0.411)(37,0.417)(38,0.423)(39,0.429)(40,0.434)(41,0.440)(42,0.445)(43,0.450)(44,0.455)(45,0.459)(46,0.464)(47,0.469)(48,0.473)(49,0.477)(50,0.481)(51,0.485)(52,0.489)(53,0.493)(54,0.497)(55,0.501)(56,0.504)(57,0.508)(58,0.511)(59,0.515)(60,0.518)};

% \drawsample[clrlambdamin]{(2,0.082)(3,0.070)(4,0.523)(5,0.430)(6,0.486)(7,0.484)(8,0.425)(9,0.585)(10,0.610)(11,0.589)(12,0.553)(13,0.544)(14,0.556)(15,0.608)(16,0.770)(17,0.739)(18,0.741)(19,0.702)(20,0.672)(21,0.648)(22,0.622)(23,0.600)(24,0.575)(25,0.555)(26,0.549)(27,0.606)(28,0.607)(29,0.589)(30,0.585)(31,0.568)(32,0.585)(33,0.572)(34,0.606)(35,0.589)(36,0.574)(37,0.559)(38,0.547)(39,0.555)(40,0.592)(41,0.616)(42,0.601)(43,0.587)(44,0.578)(45,0.566)(46,0.571)(47,0.620)(48,0.620)(49,0.615)(50,0.616)(51,0.606)(52,0.620)(53,0.610)(54,0.600)(55,0.613)(56,0.603)(57,0.592)(58,0.587)(59,0.579)(60,0.577)};
% \drawsample[clrlambdamean]{(2,0.161)(3,0.447)(4,0.647)(5,0.873)(6,0.792)(7,0.712)(8,0.642)(9,0.879)(10,0.939)(11,0.904)(12,0.836)(13,0.794)(14,0.777)(15,0.867)(16,0.954)(17,0.909)(18,0.881)(19,0.846)(20,0.806)(21,0.774)(22,0.743)(23,0.729)(24,0.700)(25,0.703)(26,0.889)(27,0.898)(28,0.927)(29,0.897)(30,0.888)(31,0.864)(32,0.856)(33,0.846)(34,0.887)(35,0.865)(36,0.851)(37,0.850)(38,0.870)(39,0.881)(40,0.885)(41,0.905)(42,0.891)(43,0.880)(44,0.867)(45,0.848)(46,0.842)(47,0.895)(48,0.942)(49,0.975)(50,0.973)(51,0.989)(52,1.009)(53,1.015)(54,0.998)(55,1.041)(56,1.027)(57,1.014)(58,1.004)(59,1.034)(60,1.031)};
% \drawsample[clrlambdamax]{(2,0.239)(3,0.823)(4,0.772)(5,1.315)(6,1.097)(7,0.941)(8,0.859)(9,1.173)(10,1.268)(11,1.219)(12,1.119)(13,1.043)(14,0.998)(15,1.126)(16,1.139)(17,1.078)(18,1.021)(19,0.989)(20,0.940)(21,0.899)(22,0.864)(23,0.858)(24,0.825)(25,0.852)(26,1.229)(27,1.190)(28,1.248)(29,1.206)(30,1.192)(31,1.161)(32,1.127)(33,1.121)(34,1.167)(35,1.141)(36,1.129)(37,1.141)(38,1.194)(39,1.207)(40,1.178)(41,1.195)(42,1.180)(43,1.173)(44,1.156)(45,1.130)(46,1.114)(47,1.169)(48,1.264)(49,1.336)(50,1.330)(51,1.372)(52,1.397)(53,1.420)(54,1.396)(55,1.469)(56,1.451)(57,1.435)(58,1.421)(59,1.490)(60,1.484)};
% \drawsample[clrlambdamin]{(2,0.488)(3,0.682)(4,1.217)(5,0.984)(6,1.004)(7,1.539)(8,1.446)(9,1.286)(10,1.409)(11,1.619)(12,1.571)(13,1.472)(14,1.370)(15,1.285)(16,1.243)(17,1.212)(18,1.188)(19,1.126)(20,1.076)(21,1.068)(22,1.081)(23,1.034)(24,1.089)(25,1.047)(26,1.152)(27,1.166)(28,1.159)(29,1.125)(30,1.088)(31,1.055)(32,1.028)(33,0.998)(34,0.980)(35,0.952)(36,0.951)(37,0.949)(38,0.925)(39,0.902)(40,0.888)(41,0.868)(42,0.860)(43,0.899)(44,0.881)(45,0.894)(46,0.875)(47,0.901)(48,0.921)(49,0.960)(50,0.941)(51,0.931)(52,0.925)(53,0.912)(54,0.896)(55,0.891)(56,0.876)(57,0.920)(58,0.904)(59,0.892)(60,0.882)};
% \drawsample[clrlambdamean]{(2,0.793)(3,1.301)(4,1.534)(5,1.514)(6,1.409)(7,1.947)(8,1.836)(9,1.636)(10,1.767)(11,1.777)(12,1.695)(13,1.582)(14,1.474)(15,1.380)(16,1.376)(17,1.450)(18,1.396)(19,1.419)(20,1.360)(21,1.321)(22,1.306)(23,1.268)(24,1.270)(25,1.296)(26,1.327)(27,1.321)(28,1.296)(29,1.255)(30,1.348)(31,1.309)(32,1.276)(33,1.320)(34,1.302)(35,1.274)(36,1.256)(37,1.234)(38,1.203)(39,1.173)(40,1.148)(41,1.122)(42,1.103)(43,1.124)(44,1.106)(45,1.136)(46,1.128)(47,1.149)(48,1.151)(49,1.168)(50,1.171)(51,1.201)(52,1.202)(53,1.181)(54,1.220)(55,1.204)(56,1.219)(57,1.253)(58,1.233)(59,1.218)(60,1.207)};
% \drawsample[clrlambdamax]{(2,1.097)(3,1.920)(4,1.852)(5,2.044)(6,1.814)(7,2.356)(8,2.225)(9,1.986)(10,2.125)(11,1.935)(12,1.819)(13,1.691)(14,1.579)(15,1.475)(16,1.510)(17,1.687)(18,1.604)(19,1.711)(20,1.644)(21,1.574)(22,1.531)(23,1.502)(24,1.451)(25,1.545)(26,1.501)(27,1.477)(28,1.433)(29,1.384)(30,1.609)(31,1.563)(32,1.523)(33,1.643)(34,1.625)(35,1.596)(36,1.561)(37,1.520)(38,1.480)(39,1.444)(40,1.408)(41,1.375)(42,1.345)(43,1.349)(44,1.332)(45,1.378)(46,1.380)(47,1.396)(48,1.380)(49,1.376)(50,1.402)(51,1.472)(52,1.479)(53,1.451)(54,1.543)(55,1.517)(56,1.563)(57,1.587)(58,1.562)(59,1.544)(60,1.533)};
% \drawsample[clrlambdamin]{(2,0.011)(3,0.129)(4,0.103)(5,0.447)(6,0.508)(7,0.501)(8,0.569)(9,0.517)(10,0.469)(11,0.497)(12,0.456)(13,0.427)(14,0.399)(15,0.372)(16,0.368)(17,0.419)(18,0.419)(19,0.586)(20,0.584)(21,0.557)(22,0.589)(23,0.567)(24,0.547)(25,0.560)(26,0.554)(27,0.534)(28,0.551)(29,0.532)(30,0.516)(31,0.601)(32,0.582)(33,0.633)(34,0.658)(35,0.680)(36,0.661)(37,0.648)(38,0.641)(39,0.625)(40,0.610)(41,0.618)(42,0.686)(43,0.687)(44,0.678)(45,0.733)(46,0.762)(47,0.748)(48,0.745)(49,0.734)(50,0.720)(51,0.717)(52,0.752)(53,0.747)(54,0.761)(55,0.779)(56,0.797)(57,0.787)(58,0.810)(59,0.840)(60,0.832)};
% \drawsample[clrlambdamean]{(2,0.502)(3,0.554)(4,0.421)(5,0.583)(6,0.577)(7,0.769)(8,0.835)(9,0.749)(10,0.681)(11,0.871)(12,1.530)(13,1.598)(14,1.545)(15,1.514)(16,1.458)(17,1.412)(18,1.354)(19,2.050)(20,2.072)(21,1.976)(22,2.109)(23,2.023)(24,2.061)(25,2.047)(26,1.980)(27,1.912)(28,1.900)(29,1.836)(30,1.775)(31,1.769)(32,1.836)(33,1.910)(34,1.884)(35,1.859)(36,1.869)(37,1.828)(38,1.862)(39,1.819)(40,1.774)(41,1.742)(42,1.751)(43,1.720)(44,1.712)(45,1.710)(46,1.695)(47,1.702)(48,1.717)(49,1.686)(50,1.660)(51,1.646)(52,1.647)(53,1.641)(54,1.640)(55,1.634)(56,1.621)(57,1.599)(58,1.591)(59,1.625)(60,1.677)};
% \drawsample[clrlambdamax]{(2,0.992)(3,0.979)(4,0.738)(5,0.719)(6,0.647)(7,1.037)(8,1.101)(9,0.980)(10,0.893)(11,1.244)(12,2.603)(13,2.770)(14,2.692)(15,2.655)(16,2.547)(17,2.404)(18,2.289)(19,3.514)(20,3.560)(21,3.394)(22,3.628)(23,3.479)(24,3.574)(25,3.534)(26,3.406)(27,3.289)(28,3.249)(29,3.139)(30,3.034)(31,2.937)(32,3.089)(33,3.187)(34,3.109)(35,3.039)(36,3.077)(37,3.009)(38,3.083)(39,3.013)(40,2.938)(41,2.866)(42,2.816)(43,2.753)(44,2.746)(45,2.687)(46,2.629)(47,2.656)(48,2.688)(49,2.638)(50,2.600)(51,2.575)(52,2.541)(53,2.536)(54,2.519)(55,2.490)(56,2.445)(57,2.411)(58,2.372)(59,2.410)(60,2.521)};
% \drawsample[clrlambdamin]{(2,0.003)(3,0.246)(4,0.552)(5,0.450)(6,0.490)(7,0.734)(8,0.692)(9,0.628)(10,0.655)(11,0.686)(12,0.631)(13,0.583)(14,0.645)(15,0.610)(16,0.573)(17,0.587)(18,0.554)(19,0.527)(20,0.506)(21,0.483)(22,0.560)(23,0.541)(24,0.586)(25,0.658)(26,0.639)(27,0.700)(28,0.767)(29,0.750)(30,0.738)(31,0.714)(32,0.706)(33,0.744)(34,0.752)(35,0.734)(36,0.740)(37,0.723)(38,0.711)(39,0.696)(40,0.696)(41,0.691)(42,0.687)(43,0.696)(44,0.680)(45,0.667)(46,0.654)(47,0.641)(48,0.645)(49,0.657)(50,0.646)(51,0.637)(52,0.626)(53,0.614)(54,0.605)(55,0.602)(56,0.599)(57,0.592)(58,0.586)(59,0.620)(60,0.613)};
% \drawsample[clrlambdamean]{(2,0.193)(3,0.690)(4,0.866)(5,0.709)(6,0.967)(7,1.126)(8,1.253)(9,1.196)(10,1.142)(11,1.282)(12,1.218)(13,1.192)(14,1.161)(15,1.225)(16,1.149)(17,1.145)(18,1.089)(19,1.043)(20,0.999)(21,0.967)(22,0.988)(23,0.948)(24,1.072)(25,1.090)(26,1.050)(27,1.085)(28,1.093)(29,1.061)(30,1.032)(31,1.005)(32,0.983)(33,1.019)(34,1.031)(35,1.048)(36,1.032)(37,1.007)(38,0.995)(39,1.049)(40,1.032)(41,1.033)(42,1.025)(43,1.014)(44,1.002)(45,0.999)(46,0.979)(47,1.073)(48,1.080)(49,1.158)(50,1.293)(51,1.364)(52,1.412)(53,1.387)(54,1.368)(55,1.377)(56,1.362)(57,1.346)(58,1.361)(59,1.431)(60,1.426)};
% \drawsample[clrlambdamax]{(2,0.383)(3,1.134)(4,1.180)(5,0.968)(6,1.444)(7,1.519)(8,1.814)(9,1.764)(10,1.628)(11,1.877)(12,1.805)(13,1.801)(14,1.677)(15,1.840)(16,1.725)(17,1.704)(18,1.623)(19,1.559)(20,1.492)(21,1.451)(22,1.416)(23,1.356)(24,1.558)(25,1.521)(26,1.462)(27,1.471)(28,1.420)(29,1.372)(30,1.326)(31,1.295)(32,1.260)(33,1.294)(34,1.310)(35,1.362)(36,1.324)(37,1.291)(38,1.280)(39,1.403)(40,1.368)(41,1.376)(42,1.363)(43,1.331)(44,1.323)(45,1.332)(46,1.303)(47,1.504)(48,1.516)(49,1.659)(50,1.940)(51,2.091)(52,2.199)(53,2.159)(54,2.131)(55,2.152)(56,2.125)(57,2.099)(58,2.135)(59,2.243)(60,2.238)};
% \drawsample[clrlambdamin]{(2,0.009)(3,0.527)(4,0.559)(5,0.516)(6,0.437)(7,0.376)(8,0.329)(9,0.314)(10,0.308)(11,0.285)(12,0.281)(13,0.481)(14,0.707)(15,0.696)(16,0.712)(17,0.701)(18,0.785)(19,0.760)(20,0.724)(21,0.767)(22,0.742)(23,0.847)(24,0.824)(25,0.861)(26,0.844)(27,0.821)(28,0.791)(29,0.765)(30,0.769)(31,0.746)(32,0.744)(33,0.738)(34,0.717)(35,0.730)(36,0.724)(37,0.711)(38,0.735)(39,0.721)(40,0.717)(41,0.793)(42,0.812)(43,0.793)(44,0.777)(45,0.768)(46,0.802)(47,0.850)(48,0.834)(49,0.829)(50,0.843)(51,0.828)(52,0.813)(53,0.808)(54,0.793)(55,0.798)(56,0.785)(57,0.772)(58,0.777)(59,0.766)(60,0.760)};
% \drawsample[clrlambdamean]{(2,0.844)(3,0.824)(4,0.733)(5,0.735)(6,0.726)(7,0.966)(8,0.877)(9,0.978)(10,1.074)(11,0.986)(12,0.914)(13,1.099)(14,1.152)(15,1.147)(16,1.188)(17,1.375)(18,1.360)(19,1.320)(20,1.262)(21,1.247)(22,1.340)(23,1.462)(24,1.488)(25,1.472)(26,1.428)(27,1.448)(28,1.403)(29,1.398)(30,1.367)(31,1.324)(32,1.299)(33,1.268)(34,1.245)(35,1.230)(36,1.209)(37,1.198)(38,1.188)(39,1.178)(40,1.193)(41,1.228)(42,1.238)(43,1.230)(44,1.212)(45,1.200)(46,1.202)(47,1.210)(48,1.186)(49,1.168)(50,1.160)(51,1.155)(52,1.141)(53,1.141)(54,1.145)(55,1.192)(56,1.181)(57,1.164)(58,1.153)(59,1.135)(60,1.122)};
% \drawsample[clrlambdamax]{(2,1.679)(3,1.120)(4,0.908)(5,0.954)(6,1.015)(7,1.556)(8,1.425)(9,1.642)(10,1.841)(11,1.687)(12,1.546)(13,1.717)(14,1.598)(15,1.597)(16,1.664)(17,2.049)(18,1.936)(19,1.880)(20,1.801)(21,1.728)(22,1.938)(23,2.077)(24,2.151)(25,2.083)(26,2.013)(27,2.076)(28,2.015)(29,2.032)(30,1.964)(31,1.903)(32,1.854)(33,1.799)(34,1.772)(35,1.729)(36,1.693)(37,1.685)(38,1.641)(39,1.635)(40,1.668)(41,1.664)(42,1.663)(43,1.667)(44,1.647)(45,1.633)(46,1.602)(47,1.569)(48,1.538)(49,1.508)(50,1.478)(51,1.482)(52,1.469)(53,1.474)(54,1.497)(55,1.587)(56,1.577)(57,1.557)(58,1.530)(59,1.505)(60,1.484)};

\drawlambda[very thick,clrlambdamax]\plotcommand{(2,1.937)(3,1.990)(4,2.008)(5,2.022)(6,2.032)(7,2.026)(8,2.025)(9,2.021)(10,2.015)(11,2.015)(12,2.013)(13,2.011)(14,2.011)(15,2.010)(16,2.006)(17,2.005)(18,2.006)(19,2.004)(20,2.001)(21,2.002)(22,2.001)(23,2.004)(24,2.003)(25,2.001)(26,2.001)(27,2.001)(28,2.000)(29,1.999)(30,2.000)(31,2.001)(32,2.000)(33,1.999)(34,1.998)(35,1.997)(36,1.997)(37,1.996)(38,1.996)(39,1.995)(40,1.995)(41,1.995)(42,1.994)(43,1.995)(44,1.995)(45,1.995)(46,1.995)(47,1.994)(48,1.995)(49,1.995)(50,1.996)(51,1.995)(52,1.996)(53,1.995)(54,1.996)(55,1.996)(56,1.996)(57,1.996)(58,1.995)(59,1.996)(60,1.997)};
\drawlambda[very thick,clrlambdamean]\plotcommand{(2,1.071)(3,1.157)(4,1.206)(5,1.241)(6,1.268)(7,1.282)(8,1.294)(9,1.302)(10,1.308)(11,1.315)(12,1.321)(13,1.325)(14,1.328)(15,1.331)(16,1.333)(17,1.336)(18,1.339)(19,1.340)(20,1.341)(21,1.344)(22,1.345)(23,1.349)(24,1.349)(25,1.350)(26,1.351)(27,1.352)(28,1.352)(29,1.353)(30,1.354)(31,1.355)(32,1.355)(33,1.355)(34,1.355)(35,1.356)(36,1.356)(37,1.356)(38,1.357)(39,1.357)(40,1.357)(41,1.357)(42,1.357)(43,1.358)(44,1.358)(45,1.359)(46,1.359)(47,1.359)(48,1.360)(49,1.360)(50,1.361)(51,1.361)(52,1.361)(53,1.361)(54,1.362)(55,1.362)(56,1.362)(57,1.362)(58,1.362)(59,1.362)(60,1.363)};
\drawlambda[very thick,clrlambdamin]\plotcommand{(2,0.206)(3,0.324)(4,0.403)(5,0.460)(6,0.505)(7,0.538)(8,0.563)(9,0.583)(10,0.600)(11,0.615)(12,0.628)(13,0.639)(14,0.646)(15,0.653)(16,0.660)(17,0.666)(18,0.672)(19,0.677)(20,0.681)(21,0.686)(22,0.689)(23,0.693)(24,0.696)(25,0.698)(26,0.700)(27,0.703)(28,0.704)(29,0.706)(30,0.707)(31,0.708)(32,0.710)(33,0.712)(34,0.713)(35,0.714)(36,0.715)(37,0.716)(38,0.717)(39,0.718)(40,0.719)(41,0.720)(42,0.721)(43,0.721)(44,0.722)(45,0.723)(46,0.724)(47,0.725)(48,0.725)(49,0.725)(50,0.726)(51,0.726)(52,0.727)(53,0.727)(54,0.727)(55,0.728)(56,0.728)(57,0.728)(58,0.728)(59,0.729)(60,0.729)};

